Nearest Neighbor Speculative Decoding for LLM Generation and Attribution

Large language models (LLMs) often hallucinate and lack the ability to provide attribution for their generations. Semi-parametric LMs, such as kNN-LM, approach these limitations by refining the output of an LM for a given prompt using its nearest neighbor matches in a non-parametric data store. However, these models often exhibit slow inference speeds and produce non-fluent texts. In this paper, we introduce Nearest Neighbor Speculative Decoding (NEST), a novel semi-parametric language modeling approach that is capable of incorporating real-world text spans of arbitrary length into the LM generations and providing attribution to their sources. NEST performs token-level retrieval at each inference step to compute a semi-parametric mixture distribution and identify promising span continuations in a corpus. It then uses an approximate speculative decoding procedure that accepts a prefix of the retrieved span or generates a new token. NEST significantly enhances the generation quality and attribution rate of the base LM across a variety of knowledge-intensive tasks, surpassing the conventional kNN-LM method and performing competitively with in-context retrieval augmentation. In addition, NEST substantially improves the generation speed, achieving a 1.8x speedup in inference time when applied to Llama-2-Chat 70B. Code will be released at https://github.com/facebookresearch/NEST/tree/main.

==> older_versions/intro_0518.tex <==
Large language models (LLMs) have exhibited remarkable capabilities in various natural language tasks, including question-answering~\citep{asai-etal-2022-evidentiality,kamalloo-etal-2023-evaluating}, summarization and mathematical reasoning~\citep{lewkowycz2022solving,yue2024mammoth}.
% , and multi-step planning~\cite{schick2023toolformer,selfrag}. \vic{It's a highly debated topic in the NeurIPS community regarding whether LLMs are capable of planning}
However, models solely relying on the knowledge learned during pre-training and alignment still suffer from factual inaccuracy and lack of attribution.
Semi-parametric LMs such as kNN-LM~\cite{knnlm} demonstrate the potential of complementing the language models with non-parametric knowledge through a key-value database.
Despite achieving lower perplexity in different domains~\cite{silo}, such models are found problematic in free-form generation tasks, yielding low-quality text outputs and high inference latency.
\cite{wang-etal-2023-knn} performed a study on kNN-LM and found that 1) kNN-LM tends to worsen the predictions for most tokens, and 2) the retrieval distribution is more susceptible to exposure bias and can be easily disrupted by artifacts in the generated text. Both of these problems suggest that retrieving tokens at every time step is not only computationally intensive but also breaks the generation consistency since most tokens are trivial to retrieve.    
% To mitigate this problem, multiple solutions have been proposed, including supervised fine-tuning~\cite{tian2024finetuning}, retrieval augmentation~\cite{ralm}, and inference-time revision~\cite{rarr}.
% However, these solutions still do not guarantee to provide accurate and consistent attributions to the generation.

\begin{figure}[t!]
\centering
\hspace{-15mm}
\begin{subfigure}[b]{0.4\textwidth}
 \centering
 \includegraphics[width=\textwidth]{nest_demo-1.pdf}
 \caption{LM: Hallucination.}\label{fig:comparison:llm}
\end{subfigure}
\hspace{-15mm}
\begin{subfigure}[b]{0.4\textwidth}
 \centering
 \includegraphics[width=\textwidth]{nest_demo-2.pdf}
 \caption{RA: Wrong attribution.}\label{fig:comparison:ra}
\end{subfigure}
\hspace{-5mm}
\begin{subfigure}[b]{0.4\textwidth}
 \centering
 \includegraphics[width=\textwidth]{nest_demo-3.pdf}
 \caption{kNN-LM: Inconsistent attribution.}\label{fig:comparison:knnlm}
\end{subfigure}
\caption{Generation and attribution of different methods. (a) LM: Non-factual output and no attribution (red). (b) In-context retrieval augmentation (RA): Factual outputs (green) but sparse and wrong attribution (red). (c) kNN-LM: Dense and correct attribution (green) but inconsistent (red).}
\label{fig:comparison}
\end{figure}

In this work, we attempt to fix the above problems in kNN-LM and make it useful for free-form generation in terms of both generation latency and quality. We introduce a solution called Nearest Neighbour Speculative Decoding (\nest) which dynamically selects consecutive segments from the corpus with post-hoc revision. \nest is a training-free, plug-and-play method that solves the consistency issues in kNN-LM generation and achieves a great balance among latency, attribution, and fluency. 
% To show the advantage of our method, we first highlight the generation issues of LLM, retrieval-augmented LLM~\cite{ralm}, and kNN-LM~\cite{knnlm} in Figure~\ref{fig:comparison}. Figure~\ref{fig:comparison:llm} demonstrates the hallucination problems in LLMs, and a common solution is to use in-context retrieval augmentation method~\cite{ralm} which first retrieves relevant passages and adds them to the prompt. The output will generally be more factual but the citation prediction does not guarantee to support the claims. On the other hand, kNN-LM gives attribution directly to each token, but it does not maintain coherence well among tokens, making the results attributable yet less factual. Moreover, due to directly incorporating non-parametric distribution into LM's prediction, kNN-LM sometimes can generate artifacts such as grammatical errors and repetition, making them less desirable for practical use.
% In contrast, 
As shown in Figure~\ref{fig:nest}, \nest improves the factuality of language model generation by providing segment-level, consistent attribution. This is achieved by its four core mechanisms summarized in the following. Each mechanism starts with the name and its purpose summarized as keywords in the parenthesis:

\noindent\textbf{Two-stage kNN search (efficiency-accuracy trade-off).} We start by breaking down the token-level datastore of kNN-LM in Section~\ref{sec:nest:two-stage}, by first creating a passage-level index and then encoding the retrieved passages into token-level key-value memory on the fly. This step is for latency-accuracy trade-off since creating the token datastore for the entire corpus is expensive using LLMs. It also acts as a filter to remove irrelevant passages with similar segments.

\noindent\textbf{Confidence-based interpolation (adaptive interpolation).} We design {Relative Retrieval Confidence} (RRC) in Section~\ref{sec:nest:rrc} to measure the uncertainty of the retriever and use it as the interpolation coefficient to aggregate the LLM's prediction and retrieval token distribution. This not only enables \nest to adapt to different queries but also guides the LM to select the appropriate tokens in the corpus instead of just from vocabulary.

\noindent\textbf{Dynamic span selection (attribution consistency).} Inspired by Copy Generator~\citep{cog}, \nest selects a span in the corpus instead of a token at each time step. This is to ensure attribution consistency such that the consecutive tokens come from the same source, described in Section~\ref{sec:nest:span}.

\noindent\textbf{Relaxed speculative decoding (fluency-attribution trade-off).} Despite providing direct and consistent attribution to the output, the mixed generation of retrieval and LLM's predictions might contain some artifacts such as repetition and grammatical errors. To ensure fluency in a training-free setting, we take inspiration from speculative decoding and use its relaxed version to reject discontinuous segments while keeping the consistent facts retrieved from the corpus in Section~\ref{sec:nest:rejection}.

Experiments of applying Llama-2-chat on various free-form generation tasks, including question answering, text completion, and fact verification, show that \nest is able to outperform the base LM and kNN-LM under a zero-shot setting. \nest is able to further combine with the in-context retrieval-augmentation method, and the mixed version enjoys the merits of both approaches (i.e., being more factual and having consistent attribution). In addition, by generating multiple tokens at each time step, \nest is able to further improve the latency of long-form generation without sacrificing attribution and fluency, achieving a 1.8x speedup in inference time for the 70B model.
